Making Large Language Models Perform Better in Knowledge Graph Completion

Large language model (LLM) based knowledge graph completion (KGC) aims to predict the missing triples in the KGs with LLMs. However, research about LLM-based KGC fails to sufficiently harness LLMs' inference proficiencies, overlooking critical structural information integral to KGs. In this paper, we explore methods to incorporate structural information into the LLMs, with the overarching goal of facilitating structure-aware reasoning. We first discuss on the existing LLM paradigms like in-context learning and instruction tuning, proposing basic structural information injection approaches. Then we propose a Knowledge Prefix Adapter (KoPA) to fulfill this stated goal. The KoPA uses a structural pre-training phase to comprehend the intricate entities and relations within KGs, representing them as structural embeddings. Then KoPA communicates such cross-modal structural information understanding to the LLMs through a knowledge prefix adapter which projects the structural embeddings into the textual space and obtains virtual knowledge tokens positioned as a prefix of the input prompt. We conduct comprehensive experiments and provide incisive analysis concerning how the introduction of cross-modal structural information would be better for LLM's factual knowledge reasoning ability. Our code and data are available at https://github.com/zjukg/KoPA .

==> chapters/7-limits_ethics.tex <==
\section*{Limitations}
In this paper, we focus on the topic of LLM-based KGC, aiming to integrate the KGC capability into LLM with structure-aware reasoning ability.
There are some limitations in our work.

\noindent \textbf{Model Design.} The design of the knowledge prefix adapter is relatively simple. A more sophisticated and subtle design will be our future plan. 

\noindent \textbf{Task Generalization.} we have not generalized the model method to all kinds of KGC tasks such as link prediction. The main task of the current research is triple classification. 


\noindent \textbf{Model Interpretability.} More in-depth experiments need to be further conducted to explore the interpretability of our model..

\section*{Ethical Considerations}
The data and pre-trained LLMs we use in our paper are all existing open-sourced resources for academic research and there are no ethical issues in our paper. We promise that there is no anti-ethic behavior in our research.

==> chapters/8.1-relatedworks.tex <==
\section{Related Works}
In this section, we add some related works about KG and LLM that for reasons of space could not be mentioned in the main paper.
\subsection{Knowledge Graph Completion}
Depending on the design of the scoring function, embedding-based methods can be divided into three sub-categories: (1) translation-based methods like TransE \cite{DBLP:conf/nips/TransE} and RotatE \cite{DBLP:conf/iclr/RotatE}, (2) tensor decomposition methods like DistMult \cite{DBLP:journals/corr/DistMult} and ComplEx \cite{DBLP:conf/icml/ComplEx}, (3) neural network-based methods like ConvE \cite{DBLP:conf/dsaa/ConvE}. Embedding-based KGC methods learn the structural embeddings for triple discrimination but neglect the textual information in the KG.

KG-BERT \cite{DBLP:journals/corr/KG-BERT} is the first PLM-based method that models KGC as a binary text classification task. Subsequent works like MTL-KGC \cite{DBLP:conf/coling/MTL-KGC} and StAR \cite{DBLP:conf/www/STAR} have further improved KG-BERT by introducing more training tasks such as relation classification and triple ranking and more complex triple encoding strategy. PKGC \cite{DBLP:conf/acl/PKGC} utilizes manual prompt templates to capture the triple semantic. Other methods like KGT5 \cite{DBLP:conf/acl/KGT5} and KG-S2S \cite{DBLP:conf/coling/KGS2S} make a step on the generative KGC \cite{DBLP:conf/emnlp/GKGC} in a sequence-to-sequence paradigm with encoder-decoder PLMs like T5 \cite{DBLP:journals/jmlr/T5}. PLM-based methods leverage the power of PLM but make the training process into text-based learning, which is difficult to capture complex structure information in the KGs.

\subsection{LLMs for KG research}
In recent years, large language models (LLMs) \cite{DBLP:journals/corr/gpt4,DBLP:conf/iclr/chatglm,DBLP:journals/corr/llama} have made rapid progress and demonstrated powerful capabilities in a considerable number of text-related tasks \cite{DBLP:journals/corr/llmsurvey}. LLMs are usually pre-trained in an auto-regressive manner with next word prediction task \cite{DBLP:conf/nips/gpt3} and demonstrate strong capability on text comprehension and generation. Some significant techniques such as instruction tuning (IT) \cite{DBLP:conf/nips/instructgpt} and human preference alignment \cite{DBLP:journals/corr/alignment} are further applied to guide the model to follow human instructions and generate responses that are consistent with human values and preferences.


\subsection{Incorporate Non-textual Modality Information into LLMs}

As LLMs demonstrate generalizable capabilities on text generation, many other works attempt to incorporate non-textual modality such as images \cite{DBLP:journals/corr/llava,DBLP:journals/corr/minigpt4}, audio \cite{DBLP:journals/corr/macaw-gpt}, and video \cite{DBLP:journals/corr/macaw-gpt}, which are also called multi-modal LLMs \cite{DBLP:journals/corr/mllm-survey}. These methods tend to encode non-textual information through the modality encoders and then process it as virtual text tokens. The non-textual tokens are aligned with the word tokens by instruction tuning on multi-modal datasets.
\par The multi-modal LLM mentioned above usually excludes graph, which is another important data modality. There are also some works talking about how to incorporate graph data into LLMs. Drug-Chat \cite{DBLP:journals/corr/druggpt} proposes to encode the drug molecule graphs with 
graph encoders and fine-tune the LLM to predict drug interactions. Other works \cite{DBLP:journals/corr/graph-llm1,DBLP:journals/corr/graph-llm2, DBLP:journals/corr/graph-llm3,DBLP:journals/corr/graph-llm4} explore how to solve graph learning tasks like node classification and graph classification by convert the graph structure information into LLMs.
\par Our research is relative to this topic as KGs also have complex graph structures on top of the text descriptions. In this paper, we will explore how to incorporate complex structural information in the KGs into the LLMs to achieve better reasoning capabilities on knowledge graph completion.


==> chapters/8.2-baselines.tex <==
\section{Base Paradigms for LLMs to Solve KGC tasks}

\subsection{Training-free Reasoning Approaches}
Training-free reasoning is an efficient approach to employing a LLM to solve downstream tasks without extra training. We need to prepare a suitable prompt template to acquire the results generated by the model $\mathcal{M}$. Mainstream training-free approaches consist of zero-shot reasoning and in-context learning \cite{DBLP:journals/corr/icl-survey}. Existing methods like \cite{DBLP:journals/corr/llm4kgc-zhu} have tried zero-shot reasoning to evaluate the link prediction ability of LLM. Besides, there are no ICL-based KGC methods yet.
We will discuss each of them below more systematically and incorporate structural information into LLMs.
\subsubsection{Zero-shot Reasoning Approach}
\label{method::zsr}
Zero-shot reasoning (ZSR) is a direct approach for LLMs to do the reasoning task without auxiliary information $\mathcal{U}$. Thus, the input sequence of ZSR can be denoted as $\mathcal{S}_{zsr}=\mathcal{I}_{zsr}\oplus\mathcal{X}$. The decoding process of the LLM $\mathcal{M}$ can be formulated as:
\begin{equation}
\begin{aligned}
    \label{zsr}
\mathcal{A}_{zsr}&=\arg\max_{\mathcal{A}}P_{\mathcal{M}}(\mathcal{A}|\mathcal{S}_{zsr})
\\&=\arg\max_{\mathcal{A}}P_{\mathcal{M}}(\mathcal{A}|\mathcal{I}_{zsr},\mathcal{X})
\end{aligned}
\end{equation}
where $\mathcal{A}$ is the generated answer of the model $\mathcal{M}$ and $\mathcal{I}_{zsr}$ is the instruction template for ZSR. In the setting of ZSR, no KG information is added to the input sequence $\mathcal{S}_{zsr}$. 
\par The determinative information in the ZSR prompt is only the textual descriptions of the test triple. ZSR is unable to incorporate KG information due to its setting limitations, otherwise, it cannot be called zero-shot. 
\subsubsection{In-context Learning Approach with Structure-aware Demonstration}
\label{method::icl}
As another training-free paradigm, in-context learning (ICL) \cite{DBLP:journals/corr/icl-survey} allows the model $\mathcal{M}$ to add auxiliary demonstration $\mathcal{U}$ to the input $\mathcal{S}$ and accomplish the task in the form of analogical reasoning, which can be denoted as:

\begin{equation}
\begin{aligned}
\mathcal{A}_{icl}&=\arg\max_{\mathcal{A}}P_{\mathcal{M}}(\mathcal{A}|\mathcal{S}_{icl})\\&=\arg\max_{\mathcal{A}}P_{\mathcal{M}}(\mathcal{A}|\mathcal{I}_{icl},\mathcal{U},\mathcal{X})
\end{aligned}
\end{equation}
\par As for the triple classification task, the demonstration $\mathcal{U}$ should be some triples and their labels in the form of $\{(\mathcal{X}_i, y_i), 1\leq i\leq k\}$, where $\mathcal{X}_i$ is the demonstration triple and $\mathcal{y}_i$ is the label. We denote the ICL with $k$ demonstrations as $k$-shot ICL.

\par The demonstration triples can be randomly sampled from the existing training KG. However, to further incorporate the relative KG information of the test triple $(h, r, t)$, we propose to sample 
triples that are in the local structure of $h$ and $t$, which means 
one of the entities in each sampled triple should be $h$ or $t$. Besides, as existing KG only consists of positive triples, we employ negative sampling \cite{DBLP:conf/acl/PKGC} to sample negative triples for demonstration. The number of positive and negative triples are the same for balanced predictions. In the demonstration prompt, the positive triples are labeled as true and the negative triples are labeled as false.
\par By doing this, we incorporate the local structural information into the demonstration prompt $\mathcal{U}$ with both positive and negative samples. Such a structure-aware demonstration could better enhance the analogical reasoning process of the model $\mathcal{M}$.

\subsection{Instruction Tuning Approaches}
Instruction tuning (IT) aims to fine-tune the LLM to follow human instructions and accomplish the mentioned tasks in the instruction prompt. In this section, we will talk about how to incorporate the KG information into IT approaches.
\subsubsection{Vanilla Instruction Tuning}
\label{method::it}
In the setting of vanilla IT, the instruction prompt $\mathcal{I}_{it}$ will describe the details of completing the triple classification task and the triple prompt $\mathcal{X}$ consists of the input triple. No other auxiliary demonstrations are included in the input template. To train the model $\mathcal{M}$, the input sequence is organized as $\mathcal{S}_{it}=\mathcal{I}_{it}\oplus\mathcal{X}\oplus\mathcal{A}_{it}$.
where $\mathcal{A}_{it}$ is the predicted answer of the training data. The model $\mathcal{M}$ is fine-tuned with the next word prediction task \cite{DBLP:journals/corr/llmsurvey} which is a universal approach to training LLMs. The training objective can be formulated as:
\begin{equation}
    \mathcal{L}_{it}=-\frac{1}{|\mathcal{S}_{it}|}\sum_{i=1}^{|\mathcal{S}_{it}|}\log P_{\mathcal{M}}(s_i|s_{<i})
\end{equation}
where $s_i(i=1,2,\dots,|\mathcal{S}_{it}|)$ represents the textual tokens of the input sequence $\mathcal{S}_{it}$. In the inference stage, the model $\mathcal{M}$ is employed to predict the answer $\mathcal{A}_{it}$ of the test data like Equation \ref{zsr}. Besides, negative sampling \cite{DBLP:conf/acl/PKGC} is also applied as training KG only consists of positve triples.
\par Vanilla IT only fine-tunes the LLM to learn the knowledge in the single triple to discriminate. Such an approach makes it difficult to fully utilize the rich semantics present in a KG and the model performance is limited.

\subsubsection{Structure-aware Instruction Tuning}
\label{method::sit}
As mentioned before, the structural information of KG plays a significant role in the KGC tasks \cite{DBLP:journals/tkde/kg-urvey}. To incorporate such KG information during the fine-tuning stage, we achieve this goal by adding the neighborhood descriptions of the input triple. Specifically, we can sample the neighborhoods of the head $h$ and tail $t$ and put the textual descriptions of neighborhood triples in the demonstration prompt $\mathcal{U}_{it}$. In this way, the input training sequence is enhanced as $\mathcal{S}_{it}=\mathcal{I}_{it}\oplus\mathcal{U}_{it}\oplus\mathcal{X}\oplus\mathcal{A}_{it}$.

We name such an approach as structure-aware instruction tuning as the local structural information of the entities is added into the input sequence in the form of neighborhood triples.




\subsection{Comparasions Among Baselines and KoPA}

We make a comparasion table of the base paradigms and KoPA, presented in Table \ref{complexity}.
\input{chapters/4.3-table}

==> chapters/8.3-experiments.tex <==
\section{Experiments}
\subsection{Dataset Details}

\begin{table}[]
\caption{Statistical information of datasets. The positve (+) and negative (-) samples are 1:1 in the valid and test set.}
\label{table::dataset}
\centering
\resizebox{\columnwidth}{!}{
\begin{tabular}{c|ccccc}
\toprule
Dataset   & $|\mathcal{E}|$    & $|\mathcal{R}|$   & \#Train & \#Valid(+/-) & \#Test(+/-) \\ \midrule
UMLS & 135 & 46 & 5216  & 652/652   & 661/661  \\
CoDeX-S   & 2034 & 42  & 32888   & 1827/1827    & 1828/1828   \\
FB15K-237N    & 13104 & 93  & 87282   &  7041/7041   & 8226/8226   \\
\bottomrule
\end{tabular}}
\end{table}

\par UMLS \cite{DBLP:journals/corr/KG-BERT} is a classic medical knowledge graph including general knowledge about medicine and health care. CoDeX-S \cite{DBLP:conf/emnlp/CoDEX} is an encyclopedic KG extracted from Wikidata \cite{DBLP:journals/cacm/wikidata}. FB15K-237N proposed in \cite{DBLP:conf/acl/PKGC} is modified from FB15K-237. Besides, CoDeX-S and FB15K-237N mine hard negative triples for a more challenging evaluation and avoid false negative samples in the validation/test dataset during dataset construction. We constructed negative samples for UMLS in the same method.

Our dataset selection is based on three key perspectives:

\par (1). \textbf{Dataset prevalence}. The three KG datasets in our experiments are all mainstream public datasets, which are widely acknowledged and extensively employed in KG-related research.
\par (2). \textbf{Dataset size}. We intentionally varied the dataset sizes, ranging from small (UMLS) to medium (CoDeX-S) to large (FB15K-237N), to explore the generalizability of our approach across datasets of different scales.
\par (3). \textbf{Dataset diversity}. Our choice also takes into account the diversity of the dataset. UMLS is a domain-specific KG dataset with substantial medical knowledge, while CoDeX-S and FB15K-237N are then two encyclopaedic KG datasets, offering a balance between general world knowledge and specialized domains.

\par From the experimental results, our method shows some improvement in all three datasets, which indicates the generality of our method.

\subsection{Baseline Details}

The specific models used for these baselines are listed below:

\par (1). \textbf{Embedding-based KGC methods}. We select four traditional embedding-based KGC methods for comparisons, namely TransE \cite{}, DistMult \cite{DBLP:journals/corr/DistMult}, ComplEx \cite{DBLP:conf/icml/ComplEx}, and RotatE \cite{DBLP:conf/iclr/RotatE}. These methods predict the triple plausibility by the learned structural embeddings and the score functions defined in the model.

\par (2). \textbf{PLM-based KGC methods}. We select KG-BERT \cite{DBLP:journals/corr/KG-BERT} and PKGC \cite{DBLP:conf/acl/PKGC} as PLM-based KGC baselines, which are classic methods focusing on the triple classification task. These methods treat triple classification as a binary text classification task.

\par (3). \textbf{LLM-based KGC methods}. LLM-based KGC research is still at an early stage. There are only KGLLaMA \cite{DBLP:journals/corr/kgllama} to be the LLM-based KGC baseline. In addition to KGLLaMA, the methods proposed in Section \ref{section3} by us including ZSR, ICL, IT, and structure-aware IT (enhanced IT) will also serve as baselines.

\subsection{Implementation Details for Baselines}
\par For embedding-based KGC methods, we reproduce the results with OpenKE
we set the embedding dimension $d_e=d_r=512$ and sample $K=32$ negative samples during training. The margin $\gamma$ is tuned among $\{0, 4, 6, 8, 12\}$. After training KGC models, we search for the best classification score threshold on the validation set for test data following the traditional setting \cite{DBLP:conf/nips/TransE}.
\par For PLM-based methods, the backbone model for PLM-based KGC methods is BERT \cite{DBLP:conf/naacl/BERT}. We fine-tune the KG-BERT according to the official code implementation. Since PKGC requires a lot of manual work to annotate each relation with a prompt, we only report the results of FB15K-237N shown in the original paper.

\par For zero-shot reasoning, in addition to measuring with the same backbone Alpaca, we also test the performance of the \textit{GPT-3.5-turbor} which has 175B parameters.
For the in-context learning method, we sample k-shot (k=1,2,4,8) structure-aware demonstrations. Besides, we sample 4 neighborhood triples for each triple to conduct structure-aware instruction tuning. For {\model}, we employ RotatE \cite{DBLP:conf/iclr/RotatE} and the score function of structural embedding pre-training and the embedding dimension is set to 512 and the adapter is a 512$\times$4096 linear projection layer.

\subsection{Training Efficiency}
\label{appendix::efficiency}
\par We would like to emphasize the notable distinction between structural embedding pre-training and the pre-training methods applied in language models (such as BERT, GPT, and LLaMA), as mentioned in our paper. Language model pre-training is conducted on the massive corpus in a self-supervised manner with transformer models which is computationally expensive. However, structural embedding pre-training is performed on a certain KG and the embedding parameters and complexity is relatively modest compared with language models. 

\par For each individual experiment, we use one A800 GPU with 80G of memory for both training and inference. Our linux server has ubuntu installed and three A800 GPUs are available, this is our detailed equipment situation. To provide more precise insight, our pre-training process takes only about ten minutes on a single A800 GPU, whereas the LLM fine-tuning process takes serveral hours for various datasets (1 hour for UMLS, 3-4 hours for CoDeX-S, 8-9 hours for FB15K-237N). Pre-training a language model like BERT and GPT requires dozens of GPUs and days of training. The discernible contrast in efficiency between these two pre-training methodologies underscores the lightweight nature of structural embedding pre-training.

\subsection{Common Ability Study}

\begin{table}[]
\caption{The specific domains in MMLU which LLM achieves higher scores after training on UMLS.}
\label{table::umls}
\begin{tabular}{c|cc}
\toprule
    & \textbf{w/o Training} & \textbf{w/ Training} \\
\midrule
Clinical & 44.9      & \textbf{47.9}  \\
\midrule
\begin{tabular}[c]{@{}c@{}}College\\ Medicine\end{tabular}   & 30.1      & \textbf{31.2}  \\
\midrule
\begin{tabular}[c]{@{}c@{}}High School\\ Biology\end{tabular}   & 42.9      & \textbf{46.8}  \\
\midrule
\begin{tabular}[c]{@{}c@{}}High School\\ Chemistry\end{tabular} & 30.0      & \textbf{32.0}  \\
\midrule
\begin{tabular}[c]{@{}c@{}}Medical\\ Genetics\end{tabular}   & 44.0      & \textbf{48.0}  \\
\bottomrule
\end{tabular}
\end{table}

We list some of the specific domains that LLMs have improved after training on the UMLS as shown in Table \ref{table::umls}.

